A lattice on decreasing trees : the metasylvester lattice

We introduce a new combinatorial structure: the metasylvester lattice on decreasing trees. It appears in the context of the $m$-Tamari lattices and other related $m$-generalizations. The metasylvester congruence has been recently introduced by Novelli and Thibon. We show that it defines a sublattice of the $m$-permutations where elements can be represented by decreasing labelled trees: the metasylvester lattice. We study the combinatorial properties of this new structure. In particular, we give different realizations of the lattice. The $m$-Tamari lattice is by definition a sublattice of our newly defined metasylvester lattice. It leads us to a new realization of the $m$-Tamari lattice, using certain chains of the classical Tamari lattice.

==> figures/binary/T3-1-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/binary/T3-1.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\node (N000) at (0.250, -1.000){};
\draw[Point] (N000) circle;
\draw (N00.center) -- (N000.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/binary/T3-2-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/binary/T3-2.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.250, -0.500){};
\node (N001) at (0.750, -1.000){};
\draw[Point] (N001) circle;
\draw (N00.center) -- (N001.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/binary/T3-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/binary/T3-3.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (1.250, -0.500){};
\node (N010) at (0.750, -1.000){};
\draw[Point] (N010) circle;
\draw (N01.center) -- (N010.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/binary/T3-4-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/binary/T3-4.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (0.750, 0.000){};
\node (N00) at (0.250, -0.500){};
\draw[Point] (N00) circle;
\node (N01) at (1.250, -0.500){};
\draw[Point] (N01) circle;
\draw (N0.center) -- (N00.center);
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/binary/T3-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/binary/T3-5.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (0.750, -0.500){};
\node (N011) at (1.250, -1.000){};
\draw[Point] (N011) circle;
\draw (N01.center) -- (N011.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}
